A framework for rigorous computational methods using Haar wavelets for differential equations

This work presents a framework for a-posteriori error-estimating algorithms for differential equations which combines the radii polynomial approach with Haar wavelets. By using Haar wavelets, we obtain recursive structures for the matrix representations of the differential operators and quadratic nonlinearities, which can be exploited for the radii polynomial method in order to get error estimates in the $L^2$ sense. This allows the method to be applicable when the system or solution is not continuous, which is a limitation of other radii-polynomial-based methods. Numerical examples show how the method is implemented in practice.

==> images/Area_under_curve.tex <==
\begin{tikzpicture}
    % Draw axis
    \draw[->,very thin] (-1,-1) -- (-1,4.5) node[anchor=west]{\color{black} \footnotesize $u$};
    \draw[->,very thin] (-2,0) -- (5,0) node[anchor=north]{\color{black} \footnotesize $t$};
    
    % Draw colored areas
    \fill[color=blue!10] (0.5,0) -- (0.5,0.5) -- (2,2) -- (2,0) -- cycle;
    \fill[color=red!10] (2,0) -- (2,2) -- (3.5,3.5) -- (3.5,0) -- cycle;
    
    % Put text inside colored areas
    \node at (1.25,0.5) {$A_1$};
    \node at (2.75,1.25) {$A_2$};
    
    % Draw dashed lines
    \draw[dashed,gray] (0.5,0) node[anchor=north]{\color{black} \footnotesize $\frac{n}{2^J}$} -- (0.5,0.5) -- (-1,0.5) node[anchor=east]{\color{black} \footnotesize $w_{jk}(\frac{n}{2^J})$};
    \draw[dashed,gray] (2,0) node[anchor=north]{\color{black} \footnotesize $\frac{n+0.5}{2^J}$}-- (2,2) -- (-1,2) node[anchor=east]{\color{black} \footnotesize $w_{jk}(\frac{n}{2^J})$};
    \draw[dashed,gray] (3.5,0) node[anchor=north]{\color{black} \footnotesize $\frac{n+1}{2^J}$} -- (3.5,3.5) -- (-1,3.5)node[anchor=east]{\color{black} \footnotesize $w_{jk}(\frac{n}{2^J})$};
    
    % Draw coarse integral
    \draw[thick] (-1,0) node[anchor=north east]{\color{black} \footnotesize $0$} -- (0,0) -- (4,4) -- (4.5,3.5);
\end{tikzpicture}

==> images/Support_overlap_coarse_wavelet.tex <==
% \begin{subfigure}{0.31\textwidth}
%     \centering
%     \begin{tikzpicture}
%         % Draw axis
%         \draw[->,very thin] (-0.5,-2) -- (-0.5,2);
%         \draw[->,very thin] (-1,0) -- (3,0);
        
%         % Draw coarse wavelet
%         \draw[dashed,blue!70] (0.5,0) -- (0.5,1.5);
%         \draw[thick,blue!70] (0.493,1.5) -- (1.507,1.5);
%         \draw[dashed,blue!70] (1.5,1.5) -- (1.5,0);
%         \draw[dashed,blue!70] (1.5,-1.5) -- (1.5,0);
%         \draw[thick,blue!70] (1.493,-1.5) -- (2.507,-1.5);
%         \draw[dashed,blue!70] (2.5,-1.5) -- (2.5,0);
        
%         % Draw fine integral
%         \draw[thick] (-1,0) -- (-0.25,0) -- (0,1) -- (0.25,0)  -- (2.9,0);
%     \end{tikzpicture}
%     \caption{Disjoint supports}
%     \label{fig:coarse_wav_fine_int_disjoint}
% \end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \centering
    \begin{tikzpicture}
        % Draw axis
        \draw[->,very thin] (-0.5,-2) -- (-0.5,2);
        \draw[->,very thin] (-1,0) -- (3,0);
        
        % Draw coarse wavelet
        \draw[dashed,blue!70] (0.5,0) -- (0.5,1.5);
        \draw[thick,blue!70] (0.493,1.5) -- (1.507,1.5);
        \draw[dashed,blue!70] (1.5,1.5) -- (1.5,0);
        \draw[dashed,blue!70] (1.5,-1.5) -- (1.5,0);
        \draw[thick,blue!70] (1.493,-1.5) -- (2.507,-1.5);
        \draw[dashed,blue!70] (2.5,-1.5) -- (2.5,0);
        
        % Draw fine integral
        \draw[thick] (-1,0) -- (0.75,0) -- (1,1) -- (1.25,0)  -- (2.9,0);
    \end{tikzpicture}
    \caption{$\text{supp }\psi_{jk}$ in $1^{\text{st}}$ half of $\text{supp }w_{Jn}$}
    \label{fig:coarse_wav_fine_int_ascend}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \centering
    \begin{tikzpicture}
        % Draw axis
        \draw[->,very thin] (-0.5,-2) -- (-0.5,2);
        \draw[->,very thin] (-1,0) -- (3,0);
        
        % Draw coarse wavelet
        \draw[dashed,blue!70] (0.5,0) -- (0.5,1.5);
        \draw[thick,blue!70] (0.493,1.5) -- (1.507,1.5);
        \draw[dashed,blue!70] (1.5,1.5) -- (1.5,0);
        \draw[dashed,blue!70] (1.5,-1.5) -- (1.5,0);
        \draw[thick,blue!70] (1.493,-1.5) -- (2.507,-1.5);
        \draw[dashed,blue!70] (2.5,-1.5) -- (2.5,0);
        
        % Draw fine integral
        \draw[thick] (-1,0) -- (1.75,0) -- (2,1) -- (2.25,0)  -- (2.9,0);
    \end{tikzpicture}
    \caption{$\text{supp }\psi_{jk}$ in $2^{\text{nd}}$ half of $\text{supp }w_{Jn}$}
    \label{fig:coarse_wav_fine_int_descend}
\end{subfigure}

==> images/Support_overlap_fine_wavelet.tex <==
% \begin{subfigure}{0.32\textwidth}
%     \centering
%     \begin{tikzpicture}
%         % Draw axis
%         \draw[->,very thin] (-0.5,-2) -- (-0.5,2);
%         \draw[->,very thin] (-1,0) -- (3,0);
%         % Draw fine wavelet
%         \draw[dashed,blue!70] (-0.25,0) -- (-0.25,1.75);
%         \draw[thick,blue!70] (-0.257,1.75) -- (0.007,1.75);
%         \draw[dashed,blue!70] (0,0) -- (0,1.75);
%         \draw[dashed,blue!70] (0,-1.75) -- (0,0);
%         \draw[thick,blue!70] (-0.007,-1.75) -- (0.257,-1.75);
%         \draw[dashed,blue!70] (0.25,-1.75) -- (0.25,0);
%         % Draw coarse integral
%         \draw[thick] (-1,0) -- (0.5,0) -- (1.5,1) -- (2.5,0)  -- (2.9,0);
%     \end{tikzpicture}
%     \caption{Disjoint supports}
%     \label{fig:fine_wav_coarse_int_disjoint}
% \end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \centering
    \begin{tikzpicture}
        % Draw axis
        \draw[->,very thin] (-0.5,-2) -- (-0.5,2);
        \draw[->,very thin] (-1,0) -- (3,0);
        % Draw fine wavelet
        \draw[dashed,blue!70] (0.75,0) -- (0.75,1.75);
        \draw[thick,blue!70] (0.743,1.75) -- (1.007,1.75);
        \draw[dashed,blue!70] (1,0) -- (1,1.75);
        \draw[dashed,blue!70] (1,-1.75) -- (1,0);
        \draw[thick,blue!70] (0.993,-1.75) -- (1.257,-1.75);
        \draw[dashed,blue!70] (1.25,-1.75) -- (1.25,0);
        % Draw coarse integral
        \draw[thick] (-1,0) -- (0.5,0) -- (1.5,1) -- (2.5,0)  -- (2.9,0);
    \end{tikzpicture}
    \caption{$\text{supp }\psi_{Jn}$ in $1^{\text{st}}$ half of $\text{supp }w_{jk}$}
    \label{fig:fine_wav_coarse_int_ascend}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
    \centering
    \begin{tikzpicture}
        % Draw axis
        \draw[->,very thin] (-0.5,-2) -- (-0.5,2);
        \draw[->,very thin] (-1,0) -- (3,0);
        % Draw fine wavelet
        \draw[dashed,blue!70] (1.75,0) -- (1.75,1.75);
        \draw[thick,blue!70] (1.743,1.75) -- (2.007,1.75);
        \draw[dashed,blue!70] (2,0) -- (2,1.75);
        \draw[dashed,blue!70] (2,-1.75) -- (2,0);
        \draw[thick,blue!70] (1.993,-1.75) -- (2.257,-1.75);
        \draw[dashed,blue!70] (2.25,-1.75) -- (2.25,0);
        % Draw coarse integral
        \draw[thick] (-1,0) -- (0.5,0) -- (1.5,1) -- (2.5,0)  -- (2.9,0);
    \end{tikzpicture}
    \caption{$\text{supp }\psi_{Jn}$ in $2^{\text{nd}}$ half of $\text{supp }w_{jk}$}
    \label{fig:fine_wav_coarse_int_descend}
\end{subfigure}
